Constraints on the Early Luminosity History of the Sun: Applications to the Faint Young Sun Problem

Stellar evolution theory predicts that the Sun was fainter in the past, which can pose difficulties for understanding Earth's climate history. One proposed solution to this Faint Young Sun problem is a more luminous Sun in the past. In this paper, we address the robustness of the solar luminosity history using the YREC code to compute solar models including rotation, magnetized winds, and the associated mass loss. We present detailed solar models, including their evolutionary history, which are in excellent agreement with solar observables. Consistent with prior standard models, we infer a high solar metal content. We provide predicted X-ray luminosities and rotation histories for usage in climate reconstructions and activity studies. We find that the Sun's luminosity deviates from the standard solar model trajectory by at most 0.5% during the Archean (corresponding to a radiative forcing of 0.849 W m$^{-2}$). The total mass loss experienced by solar models is modest because of strong feedback between mass and angular momentum loss. We find a maximum mass loss of $1.35 \times 10^{-3} M_\odot$ since birth, at or below the level predicted by empirical estimates. The associated maximum luminosity increase falls well short of the level necessary to solve the FYS problem. We present compilations of paleotemperature and CO$_2$ reconstructions. 1-D "inverse" climate models demonstrate a mismatch between the solar constant needed to reach high temperatures (e.g. 60-80 $^{\circ}$C) and the narrow range of plausible solar luminosities determined in this study. Maintaining a temperate Earth, however, is plausible given these conditions.

==> Teff.tex <==
0.0 & 4318.345 \\
0.2 & 5653.666 \\
0.4 & 5660.518 \\
0.6 & 5666.609 \\
0.8 & 5672.539 \\
1.0 & 5678.371 \\
1.2 & 5684.150 \\
1.4 & 5689.835 \\
1.6 & 5695.479 \\
1.8 & 5701.084 \\
2.0 & 5706.614 \\
2.2 & 5712.099 \\
2.4 & 5717.529 \\
2.6 & 5722.895 \\
2.8 & 5728.197 \\
3.0 & 5733.422 \\
3.2 & 5738.558 \\
3.4 & 5743.598 \\
3.6 & 5748.528 \\
3.8 & 5753.360 \\
4.0 & 5758.066 \\
4.2 & 5762.632 \\
4.4 & 5767.056 \\
4.6 & 5770.847 \\


==> luminosity.tex <==
0.0 & 20.129 \\
0.2 & 0.722 \\
0.4 & 0.734 \\
0.6 & 0.745 \\
0.8 & 0.755 \\
1.0 & 0.765 \\
1.2 & 0.776 \\
1.4 & 0.787 \\
1.6 & 0.798 \\
1.8 & 0.809 \\
2.0 & 0.820 \\
2.2 & 0.832 \\
2.4 & 0.844 \\
2.6 & 0.857 \\
2.8 & 0.869 \\
3.0 & 0.882 \\
3.2 & 0.896 \\
3.4 & 0.910 \\
3.6 & 0.924 \\
3.8 & 0.939 \\
4.0 & 0.954 \\
4.2 & 0.970 \\
4.4 & 0.986 \\
4.6 & 1.000 \\


==> properties.tex <==
0.0 & 20.141 & 7.993 & 4324.147 \\
0.2 & 0.722 & 0.885 & 5655.477 \\
0.4 & 0.734 & 0.890 & 5662.561 \\
0.6 & 0.745 & 0.894 & 5668.669 \\
0.8 & 0.755 & 0.899 & 5674.483 \\
1.0 & 0.765 & 0.903 & 5680.205 \\
1.2 & 0.776 & 0.907 & 5685.879 \\
1.4 & 0.787 & 0.912 & 5691.491 \\
1.6 & 0.798 & 0.916 & 5697.061 \\
1.8 & 0.809 & 0.921 & 5702.561 \\
2.0 & 0.820 & 0.926 & 5707.997 \\
2.2 & 0.832 & 0.931 & 5713.394 \\
2.4 & 0.844 & 0.936 & 5718.727 \\
2.6 & 0.857 & 0.941 & 5723.998 \\
2.8 & 0.869 & 0.946 & 5729.201 \\
3.0 & 0.883 & 0.951 & 5734.326 \\
3.2 & 0.896 & 0.957 & 5739.357 \\
3.4 & 0.910 & 0.963 & 5744.292 \\
3.6 & 0.924 & 0.969 & 5749.127 \\
3.8 & 0.939 & 0.975 & 5753.839 \\
4.0 & 0.954 & 0.981 & 5758.439 \\
4.2 & 0.970 & 0.988 & 5762.887 \\
4.4 & 0.986 & 0.994 & 5767.183 \\
4.6 & 1.000 & 1.000 & 5770.741 \\


==> radius.tex <==
0.0 & 8.012 \\
0.2 & 0.885 \\
0.4 & 0.890 \\
0.6 & 0.895 \\
0.8 & 0.899 \\
1.0 & 0.904 \\
1.2 & 0.908 \\
1.4 & 0.912 \\
1.6 & 0.917 \\
1.8 & 0.921 \\
2.0 & 0.926 \\
2.2 & 0.931 \\
2.4 & 0.936 \\
2.6 & 0.941 \\
2.8 & 0.946 \\
3.0 & 0.952 \\
3.2 & 0.957 \\
3.4 & 0.963 \\
3.6 & 0.969 \\
3.8 & 0.975 \\
4.0 & 0.981 \\
4.2 & 0.988 \\
4.4 & 0.994 \\
4.6 & 1.000 \\

